Practical Considerations for Discrete-Time Implementations of Continuous-Time Control Barrier Function-Based Safety Filters

Safety filters based on control barrier functions (CBFs) have become a popular method to guarantee safety for uncertified control policies, e.g., as resulting from reinforcement learning. Here, safety is defined as staying in a pre-defined set, the safe set, that adheres to the system's state constraints, e.g., as given by lane boundaries for a self-driving vehicle. In this paper, we examine one commonly overlooked problem that arises in practical implementations of continuous-time CBF-based safety filters. In particular, we look at the issues caused by discrete-time implementations of the continuous-time CBF-based safety filter, especially for cases where the magnitude of the Lie derivative of the CBF with respect to the control input is zero or close to zero. When overlooked, this filter can result in undesirable chattering effects or constraint violations. In this work, we propose three mitigation strategies that allow us to use a continuous-time safety filter in a discrete-time implementation with a local relative degree. Using these strategies in augmented CBF-based safety filters, we achieve safety for all states in the safe set by either using an additional penalty term in the safety filtering objective or modifying the CBF such that those undesired states are not encountered during closed-loop operation. We demonstrate the presented issue and validate our three proposed mitigation strategies in simulation and on a real-world quadrotor.

==> sections/experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}

==> sections/related-literature.tex <==
\section{Related Literature}
\label{sec:literature}
In this section, we provide an overview of the literature on using safety filters to certify uncertain systems under input constraints.
Safety filters are add-on modules that guarantee safety for potentially unsafe controllers, e.g., reinforcement learning agents~\cite{DSL2021}.
Generally, there exist two different types of 
safety filters: implicit safety filters and explicit safety filters. 
This distinction indicates 
% whether the safety filter leverages 
the explicit or implicit existence of a safe set. 
For discrete-time systems, model predictive safety filters~(MPSFs)~\cite{zeilinger_linear} are an example of implicit safety filters that have been used to certify uncertain systems under input constraints. MPSFs do not leverage a pre-computed safe set and typically require significant online computation.
For continuous-time systems, CBF-based safety filters~\cite{Ames2014} require explicit knowledge of a safe set. 
While the computation of such safe sets for nonlinear systems typically necessitates considerable offline computation~\cite{Dai2022}, 
the desired certificate can be efficiently determined using a quadratic program~(QP) under common assumptions~\cite{ames2019a}. 
Motivated by the goal of achieving safe real-world operation of resource-limited hardware systems, e.g., miniature quadrotors, we focus on CBF-based safety filters in this paper due to their reduced online computation. 

CBFs provide a scalar condition to determine whether a proposed control input renders a system safe on the safe set~\cite{ames2019a}.
The CBF condition is derived from Nagumo's theorem~\cite{Nagumo1942berDL}, which intuitively defines safety by guaranteeing that 
% behavior of the system at the boundary of the safe set, e.g., 
for any state on the safe set's boundary, the system will not leave the safe set. 

% 
Generally, CBFs can be synthesized by solving the Hamilton-Jacobi-Bellmann~(HJB) equations, for partially known dynamic systems~\cite{mitchell2005time, Fisac2019}. 
% For polynomial dynamics, methods involving sum of squares~(SOS) programming can be used to synthesize polynomial CBFs~\todo{(add citations)}.
% The computationally efficient synthesis of CBFs is an active field of research and often relies on the assumption of full knowledge of the system dyanmics. 
More recent methods include the more efficient solution to HJB equations, \todo{(citation)}, accounting for control input constraints in the CBF synthesis~\cite{Dai2022, Wei2023}, and leveraging deep learning methods to learn a CBF for systems with unknown dyanmics from data~\cite{Qin2022}. 

% Input constraints for CBFs
Real-world systems typically have actuation limits. For safety, these input constraints have to be accounted for. Otherwise, the assumption of additional control authority can lead to safety violations. To guarantee feasibility, the authors in~\cite{Zeng2021} propose to linearly scale the lower bound of the CBF condition online. This guarantees the feasibility of the CBF condition inside the safe set, however, the authors do not provide any guarantees on the boundary of the safe set. Another line of work, considers the case where the original safe set can no longer be rendered control invariant under input constraints and proposes to calculate subsets of the initial safe set that can be rendered safe~\cite{Agrawal2021}. 
% It does not give a recipe for creating a class $\K$ function. Rather a method for creating smaller subsets of the original desired safe set. 

% Learning and CBFs
CBFs have been combined with learning to reduce the conservatism in the safety filter design for uncertain systems~\cite{DSL2021}.  
Under the assumption of a given CBF and no input constraints, these approaches either estimate the dynamics model~\cite{Wang2018a, Ohnishi2019} or directly learn the Lie derivative~\cite{taylor2020a, l4dc22}.
%
% In~\cite{Choi2020, taylor2020a}, neural network models are used to learn the  CBF conditions offline from pre-collected data.
%
In~\cite{Wang2018a, Ohnishi2019, Castaneda2021, l4dc22}, probabilistic learning techniques for CBFs have been proposed to 
% explicitly account for the uncertainty of the learned CBF condition and 
guarantee safety of the system with high probability.

\todo{define CBF acro here}


